Interpretation of Swedish Sign Language using Convolutional Neural Networks and Transfer Learning

The automatic interpretation of sign languages is a challenging task, as it requires the usage of high-level vision and high-level motion processing systems for providing accurate image perception. In this paper, we use Convolutional Neural Networks (CNNs) and transfer learning in order to make computers able to interpret signs of the Swedish Sign Language (SSL) hand alphabet. Our model consist of the implementation of a pre-trained InceptionV3 network, and the usage of the mini-batch gradient descent optimization algorithm. We rely on transfer learning during the pre-training of the model and its data. The final accuracy of the model, based on 8 study subjects and 9,400 images, is 85%. Our results indicate that the usage of CNNs is a promising approach to interpret sign languages, and transfer learning can be used to achieve high testing accuracy despite using a small training dataset. Furthermore, we describe the implementation details of our model to interpret signs as a user-friendly web application.

==> util.tex <==
\usepackage{soul}
\usepackage{tikz}

\usetikzlibrary{calc}
\usetikzlibrary{decorations.pathmorphing}

\makeatletter

\newcommand{\defhighlighter}[3][]{%
  \tikzset{every highlighter/.style={color=#2, fill opacity=#3, #1}}%
}

\defhighlighter{yellow}{.5}

\newcommand{\highlight@DoHighlight}{
  \fill [ decoration = {random steps, amplitude=1pt, segment length=15pt}
        , outer sep = -15pt, inner sep = 0pt, decorate
        , every highlighter, this highlighter ]
        ($(begin highlight)+(0,8pt)$) rectangle ($(end highlight)+(0,-3pt)$) ;
}

\newcommand{\highlight@BeginHighlight}{
  \coordinate (begin highlight) at (0,0) ;
}

\newcommand{\highlight@EndHighlight}{
  \coordinate (end highlight) at (0,0) ;
}

\newdimen\highlight@previous
\newdimen\highlight@current

\DeclareRobustCommand*\highlight[1][]{%
  \tikzset{this highlighter/.style={#1}}%
  \SOUL@setup
  %
  \def\SOUL@preamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@BeginHighlight
      \highlight@EndHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@postamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@EndHighlight
      \highlight@DoHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@everyhyphen{%
    \discretionary{%
      \SOUL@setkern\SOUL@hyphkern
      \SOUL@sethyphenchar
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everyexhyphen##1{%
    \SOUL@setkern\SOUL@hyphkern
    \hbox{##1}%
    \discretionary{%
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everysyllable{%
    \begin{tikzpicture}[overlay, remember picture]
      \path let \p0 = (begin highlight), \p1 = (0,0) in \pgfextra
        \global\highlight@previous=\y0
        \global\highlight@current =\y1
      \endpgfextra (0,0) ;
      \ifdim\highlight@current < \highlight@previous
        \highlight@DoHighlight
        \highlight@BeginHighlight
      \fi
    \end{tikzpicture}%
    \the\SOUL@syllable
    \tikz[overlay, remember picture] \highlight@EndHighlight ;%
  }%
  \SOUL@
}

\makeatother

% Common abbrev. are set as commands to ensure proper spacing after the dot
\newcommand{\ie}{i.e.\@\xspace}
\newcommand{\aka}{a.k.a.\@\xspace}
\newcommand{\Aka}{A.k.a.\@\xspace}
\newcommand{\Ie}{I.e.\@\xspace}
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\Cf}{Cf.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}
\newcommand{\Eg}{E.g.\@\xspace}
\newcommand{\etal}{et al.\@\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\wrt}{w.r.t.\@\xspace}
\newcommand{\Wrt}{W.r.t.\@\xspace}
\newcommand{\mc}{Maven Central\@\xspace}
\newcommand{\semi}{semantic equivalence modulo inputs\@\xspace}
\newcommand{\latests}{\text{\texttt{LATESTS}\@\xspace}}
\newcommand{\pas}{\text{\texttt{P}\@\xspace}}
\newcommand{\act}{\text{\texttt{A}\@\xspace}}
\newcommand{\latest}{\text{$latest$\@\xspace}}
\newcommand{\notlatests}{\overline{\latests}}%% NOTE, it should be used in Math mode!

% List of considered decompilers
\newcommand{\krakatau}{\textsf{Krakatau}\@\xspace}
\newcommand{\jode}{\textsf{Jode}\@\xspace}
\newcommand{\cfr}{\textsf{CFR}\@\xspace}
\newcommand{\fernflower}{\textsf{Fernflower}\@\xspace}
\newcommand{\procyon}{\textsf{Procyon}\@\xspace}
%\newcommand{\jd}{\textsf{JD-GUI}\@\xspace}
\newcommand{\jd}{\textsf{JD-Core}\@\xspace}
\newcommand{\jadx}{\textsf{JADX}\@\xspace}
\newcommand{\dava}{\textsf{Dava}\@\xspace}
\newcommand{\meta}{\textsf{Multi-DC}\@\xspace}

%\newcommand{\metadc}{\textsf{MetaDecompiler}\@\xspace}
\newcommand{\metadc}{\textsf{Arlecchino}\@\xspace}


\newcommand{\javac}{\textit{javac}\@\xspace}
\newcommand{\ecj}{\textit{ecj}\@\xspace}

\newcommand{\mdg}{MDG\@\xspace}
\newcommand{\mdgl}{$\text{MDG}_L$\@\xspace}
\newcommand{\start}{\texttt{START}\@\xspace}
\newcommand{\snapshot}{\texttt{SNAPSHOT}\@\xspace}
\newcommand{\isPassive}{isPsv}
\newcommand{\orderV}{\displaystyle {<}_{v}}
\newcommand{\orderT}{\displaystyle {<}_{t}}
\newcommand{\lib}{\texttt{LIBS}\@\xspace}

% comment commands for co-authors
\newcommand{\cesar}[1]{\mynote{Cesar}{#1}}
\newcommand{\benoit}[1]{\mynote{Benoit}{#1}}
\renewcommand{\todo}[1]{\mynote{todo}{#1}}

%\newcommand{\nbartifacts}{$1,487,956$\@\xspace}
%\newcommand{\nblibraries}{$73,653$\@\xspace}
\newcommand\highlightred[1]{\colorbox{red!17}{#1}}



\newcommand{\mstore}{Fragment Store\xspace}
\newcommand{\store}{fragment store\xspace}

%\newcommand{\modified}[1]{{\color{blue}#1}} 
\newcommand{\modified}[1]{#1} 
%\newcommand\textvtt[1]{{\normalfont\fontfamily{cmvtt}\selectfont #1}}
